Rendering Anywhere You See: Renderability Field-guided Gaussian Splatting

Scene view synthesis, which generates novel views from limited perspectives, is increasingly vital for applications like virtual reality, augmented reality, and robotics. Unlike object-based tasks, such as generating 360{\deg} views of a car, scene view synthesis handles entire environments where non-uniform observations pose unique challenges for stable rendering quality. To address this issue, we propose a novel approach: renderability field-guided gaussian splatting (RF-GS). This method quantifies input inhomogeneity through a renderability field, guiding pseudo-view sampling to enhanced visual consistency. To ensure the quality of wide-baseline pseudo-views, we train an image restoration model to map point projections to visible-light styles. Additionally, our validated hybrid data optimization strategy effectively fuses information of pseudo-view angles and source view textures. Comparative experiments on simulated and real-world data show that our method outperforms existing approaches in rendering stability.

==> sec/0_abstract.tex <==

\begin{abstract}
Scene view synthesis, which generates novel views from limited perspectives, is increasingly vital for applications like virtual reality, augmented reality, and robotics. Unlike object-based tasks, such as generating 360° views of a car, scene view synthesis handles entire environments where sparse and non-uniform observations pose unique challenges for stable rendering quality. To address this issue, we propose a novel approach: renderability field-guided gaussian splatting (RF-GS). This method quantifies input inhomogeneity through a renderability field, guiding pseudo-view sampling to enhanced visual consistency. To ensure the quality of wide-baseline pseudo-views, we train an image restoration model to map point projections to visible-light styles. Additionally, our validated hybrid data optimizing strategy effectively fuses information of pseudo-view angles and source view textures. Comparative experiments on simulated and real-world data show that our method outperforms existing approaches in rendering stability.


\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}\label{sec:intro}
Rendering 3D scenes is crucial for the realization of digital twins \cite{22}. At the same time, the renewed interest in Virtual Reality/Mixed Virtual Reality (VR/MR) has further increased the demand for real-time high-fidelity rendering. Some current research results~\cite{1,2,7,8} achieve high-fidelity rendering, but the reliance on dense views prevents them from being directly applicable in practice~\cite{28}. When reconstructing realistic scenes, relying on dense inputs to achieve practical applications is usually costly~\cite{27}.


Neural Radiance Fields (NeRF)~\cite{1} represented a significant advancement in the reconstruction of objects through neural radiation field representations. Researchers have explored the integration of NeRF with volumetric rendering techniques~\cite{26}, which helped to minimize the number of required viewpoints. Subsequent studies~\cite{29,30} have employed various regularization methods to improve the generalization capabilities of new view synthesis. However, NeRF requires substantial training and rendering costs~\cite{34} to achieve high-quality results, largely due to its reliance on implicit representation methods.
\begin{figure}[t]
        \centering
	\begin{minipage}[c]{0.47\textwidth}
		\includegraphics[width=\textwidth]{sec/images/abstract-a.pdf}
		% \subcaption{GT}
		% \label{GT}
	\end{minipage}
 
	\begin{minipage}[c]{0.23\textwidth}
		\includegraphics[width=\textwidth]{sec/images/abstract-b.pdf}
		\subcaption{}
		\label{Baseline}
	\end{minipage} 
	\begin{minipage}[c]{0.23\textwidth}
		\includegraphics[width=\textwidth]{sec/images/abstract-c.pdf}
		\subcaption{}
		\label{MIXED}
	\end{minipage}

	\caption{An instance of non-uniform observation. The top figure illustrates a scenario where the viewpoint in the question mark region spans across a wide baseline, while the exclamation mark region is within the narrow baseline. (a) and (b) show synthesized views for the same region when the viewpoint is positioned in the exclamation and question mark region, respectively. }
	\label{abstract}
\end{figure}

Unlike NeRF’s implicit 3D scene representation, 3D Gaussian Splatting (GS)~\cite{2} leverages Structure-from-Motion (SfM) \cite{33} to generate a rough point cloud, representing the entire scene with Gaussian ellipses, which significantly reduces scene optimizing and rendering time. However, 3D GS depends heavily on various perspectives and is prone to overfitting in weakly observed regions, resulting in notable degradation in rendering quality~\cite{6, 34} and introducing potential reliability issues. Additionally, due to the movable range disparity between source image capture and scene visiting, even with increased shot density~\cite{31,8}, localized artifacts remain challenging to eliminate.

\begin{figure*}[htp]
\centering
\captionsetup{type=figure}
\includegraphics[width=1.0\textwidth]{sec/images/structure.pdf}
\captionof{figure}{Overall pipeline of RF-GS. Given a series of source views and the scene point cloud, our method first calculates three metrics to obtain the renderability value of each viewpoint, which is then resampled to obtain the pseudo-view. Image restoration model is trained based on the source views, and the point cloud projection of the pseudo-view is restored to visible light image during inference. Finally, 3D Gaussian primitives are refined with the mixed data, significantly alleviating rendering artifacts compared to using only ground truth.}
\label{fig:structurel}
\end{figure*}

Non-uniform observations refer to low frequency of observations and incomplete directional coverage. Figure~\ref{abstract} indicates that, under wide baseline conditions, the rendering quality in non-uniform observation regions (e.g., the ground) is significantly lower than in uniform observation regions (e.g., the leftmost table) and diverges notably from the synthesized view produced under narrow baseline conditions. To mitigate the negative effects of non-uniform inputs on the 3D GS model, we propose a renderability field-guided 3D GS approach, illustrated in Figure~\ref{fig:structurel}. The core of our method is data augmentation through pseudo-views, which strengthens the model’s generalization capabilities. 

We construct a renderability field based on the source view and the map generated from LiDAR scans, estimating the likelihood of high-quality rendering from any viewpoint within the scene. This field enables the identification of weakly observed views. In parallel, we train an image restoration model to map point-projection to visible images, transforming views sampled from the renderability field into high-quality pseudo-views. The GS model is initialized with the map and optimazation in multiple stages on hybrid data, ensuring stable rendering across the entire scene.

Our contributions can be summarized as follows.


\textbullet~We propose a renderability field-guided pseudo-view sampling method that quantifies the distribution of scene observations and enhances perspective coverage in sparsely observed regions.

 

\textbullet~We addressed the challenge of wide-baseline data augmentation by transforming geometrically consistent point-projection images into color images using an image restoration model.

\textbullet~Our extensive evaluation demonstrates the capability of the developed pipeline to effectively render challenging areas, surpassing state-of-the-art methods.

\textbullet~We discuss the limitations of current rendering quality evaluation methods for scene-oriented novel view synthesis and propose a new scheme to assess rendering stability.
%这里应该是单纯的渲染质量无法说明渲染稳定性，13说明了测试数据均匀分布在源视图，视角相似性很高，无法估计是否发生过拟合。仿真数据要说明这两点1.测试数据应该是更全面的相比较训练数据（两次FPS采样），2.测试数据的分布很重要，尽可能范围大且均匀，照顾到各个视角（FPS采样）。注：这时候测试数据保证了窄基线和宽基线的视图分布

%只要源视图分布不均匀，那么二次采样，测试数据就是均匀的，而训练数据是不均匀的，就可以测试出不均匀性，无法评估的就定性

%方法就是（对于给定的数据集，先按照一定比例用FPS采样得到测试数据，然后在相同的数据中按同样比例采样得到训练数据，由于FPS先得到稀疏分布，所以测试数据相比于训练数据的分布会更加全面（因为测试数据在密集区域和稀疏区域采样一样多，那么稀疏区域的视角就少了（而测试数据是分布均匀的），后续训练视图采样得到的结果就不均匀），存在更多的宽基线视角），再结合SDP就完全说明这个点.



% \textbullet~We make all our data and related codes publicly available to benefit the research community.





==> sec/2_related_works.tex <==
\section{Related Works}
\label{sec:formatting}

High-fidelity real-time scene rendering has become crucial for various applications, including virtual reality (VR), autonomous driving, and digital twins. This demand has driven a surge in research to enhance the quality of rendering techniques to support these rapidly evolving fields.

%-------------------------------------------------------------------------

\textbf{Scene representation.} Novel view synthesis focuses on generating novel views of a scene from a given set of images~\cite{35}. Mip-NeRF~\cite{9} improved the accuracy of high-frequency texture representations and the realism of generated images by refining the neural network structure, optimizing the loss function, and incorporating advanced and innovative training techniques. Other research efforts, including Tensorf~\cite{19}, Plenoxels~\cite{20}, and Instant-NGP~\cite{21}, have prioritized faster algorithm performance, often by reducing network complexity, employing more efficient optimization algorithms, or designing streamlined rendering pipelines. 3D GS~\cite{2} leveraged an explicit model to enable high-resolution real-time rendering. However, this effect relies on dense input data~\cite{3}; when the source views are sparse, 3D GS, like NeRF, faces challenges with generalizing well to unseen views synthesis~\cite{6}.

%-------------------------------------------------------------------------

\textbf{View dependency.} Sparse inputs, while reducing data preparation costs, increase the risk of overfitting. RegNeRF~\cite{28} addressed this by estimating underlying scene geometry errors and applying careful regularization to enhance the appearance of unobserved views, followed by optimizing the ray-sampling space with an annealing strategy and refining the colors of unseen views using a normalized flow model. Diet-NeRF~\cite{4} sought to leverage a vision-language model~\cite{5} for rendering unseen views, though the high-level semantic guidance falls short in effectively aiding low-level reconstruction. Dreamfusion~\cite{9} introduced Score Distillation Sampling (SDS), utilizing 2D priors from pre-trained diffusion models to improve scene understanding and reconstruction. Methods like DiffusioNeRF~\cite{15}, SparseFusion~\cite{16}, and ReconFusion~\cite{17} also integrated diffusion models with NeRF, though they require extensive 3D data as priors, limiting their applicability.

FSGS~\cite{34} pioneered sparse view reconstruction for 3D GS, using a 2D depth estimation network and online augmented views to guide geometric optimization, resulting in precise scene geometry reconstruction. SparseGS~\cite{6} and DNGaussian~\cite{3} similarly used a pre-trained 2D network to ensure geometric accuracy and applied SDS loss to improve new view rendering accuracy. GaussianObject~\cite{23} took a different approach by interpolating source views, employing a diffusion model-based fine-tuning model~\cite{36} to enhance pseudo-view renders, thus augmenting sparse views and improving multi-view consistency in the Gaussian splatting model. Feed-forward modeling methods~\cite{12,44,45} split sparse multi-view reconstruction into two stages: establishing a robust initialization and refining the GS model, effectively improving rendering performance under sparse inputs. However, these methods require extensive pre-training on similar-scale scenes.

\textbf{Uniform observations.} Novel view synthesis depends on the angular uniformity and frequency of observations~\cite{48}, which may not be guaranteed during scene data acquisition. Regularization-based methods typically operate with a fixed number of observations in a scene or object, limiting their flexibility and ability to adapt to non-uniformity inputs dynamically. Interpolation-based data augmentation methods are also constrained, struggling to synthesize pseudo-views under wide baselines. As a result, achieving stable rendering of arbitrary novel views with non-ideal inputs in free scenes remains challenging.

To ensure that 3D GS models can generalize across the entire scene and facilitate their utility in applications like VR, we provide three key insights. First, the renderability field effectively evaluates observation distribution, providing viewpoint-specific guidance to optimize Gaussian primitives. Second, wide-baseline pseudo-view quality can be enhanced by incorporating an image restoration model that maps the point projection image to the visible image. Lastly, scene-oriented evaluation of rendering quality should account for the algorithm's generalizability across the entire scene, which is normally constrained by test data. Therefore, we constructed intensive test cases using simulation data and preliminarily evaluated our method's performance. Additionally, we introduce the standard deviation of rendering quality to gauge an algorithm's ability to synthesize wide-baseline views in real scenes.


==> sec/3_methodology.tex <==
\section{Method}

Given a scene containing a set of $N$ source views $I=\left\{I_{i}\right\}_{i=1}^{N}$ which is corresponding to real data, camera extrinsic $T=\left\{T_{i}\right\}_{i=1}^{N}$, intrinsics $C=\left\{C_{i}\right\}_{i=1}^{N}$, and a point cloud map $M$ obtained by the composition and merging of multiple LiDAR scans unified in its coordinate system, our goal is to sample pseudo-views $I_{p}$ through the renderability field to supplement the wide baseline views. This process yields a 3D Gaussian model $M_{g}$, capable of generalizing to any view through optimization based on the hybrid data, thereby maintaining global rendering stability.

\subsection{Renderability Field Construction}\label{RFC}
The renderability field predicts the rendering quality for any viewpoint within the movable range of the reconstructed target and automatically identifies and prioritizes views that require enhancement.

\textbf{Intensive Sampling.} Benefiting from the point cloud map, we can specify viewpoint sampling intervals with a realistic scale. To ensure a comprehensive evaluation of complex indoor scenes, we perform voxel sampling within the bounding box of the environment. Given the bounding box \( B \) with maximum coordinates \( B_{\text{max}} \) and minimum coordinates \( B_{\text{min}} \), and a uniform sampling interval \( S \) along any axis, the set of viewpoints \( \boldsymbol{P_v} \) can be expressed as:

\begin{equation}\label{view sampling}
\begin{split}
\boldsymbol{P_v} = \big\{ (x, y, z) \mid\, & x = B_{\text{min},x} + iS, \\
                                  & y = B_{\text{min},y} + jS, \\
                                  & z = B_{\text{min},z} + k\frac{S}{2}, \\
                                  & i, j, k \in \mathbf{Z}, \, \text{and} \, (x, y, z) \in B \big\}.
\end{split}
\end{equation}



Since the source views are more centrally distributed on the Z-axis, we increased the sampling density on that axis. For each viewpoint, we generate six outward viewing directions to the positive and negative axes along $x$,$y$, and $z$, thus achieving a full 360-degree  observation, ensuring a comprehensive renderability assessment. 
.


\textbf{Source Images Calculation.} To compute the metrics, We need to confirm the source view sequence for each point in the point cloud map. Given the pose of real-world capture \( T = \{R, t\} \) and intrinsic parameters \( K \), we project the 3D points onto the image plane, thus constructing a set of pixel values and corresponding image indices for each 3D point. The projection equations are as follows:

\begin{equation}\label{source_img}
\left\{
\begin{array}{l}
p' = K (Rp + t),\\
P(p, T, K) = \left( \frac{p'_x}{p'_z}, \frac{p'_y}{p'_z} \right).
\end{array}
\right.
\end{equation}

Here, \( p \) is a point in 3D space, \( R \) is the world-to-camera rotation matrix, \( t \) is the translation vector, \( K \) is the intrinsic parameter matrix, \( p' \) are the projected pixel coordinates, and \( P(p, T, K) \) represents the image plane coordinates of point \( p \) given the pose \( T \) and intrinsic parameters \( K \).


\begin{figure}[!htp]
\centering
\includegraphics[width=0.45\textwidth]{sec/images/invalid_view.pdf}
\caption{Observation conflict issue. The point cloud represents only the internal structure of the scene, while the pseudo-view observes the exterior to establish a relationship with the source view through co-visible regions. However, since no source view observes this exterior region, it is a false co-visible area.}
\label{fig_7}
\end{figure}
\textbf{Observation Conflict Judgement.} Not all viewpoints are valid: some are too close to the point cloud, while others lie outside the coverage of the source views. As shown in Figure~\ref{fig_7}, since they do not establish a correct light reflection relationship with the source view, calculating the renderability value is unnecessary. To minimize the computation of irrelevant viewpoints, we implemented a filtering strategy to exclude them. If a pseudo-viewpoint has no unidirectional observation with any source viewpoints, it is in an unobserved area. We identify unidirectional observations through grid collision detection: for each pseudo-viewpoint, we first obtain the set of source views observed by its point cloud, then voxelize the sub-map determined by the pseudo-viewpoint. By linearly interpolating a series of 3D points along the line connecting the pseudo-viewpoint and the source viewpoints, and checking whether these virtual positions (including the endpoints) lie inside the voxels, we determine if there is an occlusion between the viewpoints. Additionally, we ensure that the pseudo-viewpoint maintains an appropriate distance from the scene geometry.



\textbf{Renderability Estimation.} We estimate the renderability based on the principles of Image-Based Rendering (IBR). We introduce resolution, angular, and geometric metrics as proposed in previous work~\cite{41}. For any 3D point $p$ within a pseudo-view $I^i_p$, the geometric metric is represented by the average photometric difference between source views after normalizing the colors.
\begin{equation}\label{eq1}\left.H^p_{geo}=\left\{\begin{array}{ll}1-\frac{\sum_{v_i,v_j\in \boldsymbol{I_s},i\neq j}||c(v_i,p)-c(v_j,p)||_2}{\sqrt{3} \cdot \frac{N \cdot (N-1)}{2}},&N > 1,\\1,&N \leq 1.\end{array}\right.\right.\end{equation}

Here, $N$ denotes the number of source views $\boldsymbol{I_s}$ for point $p$, and $c(v_i,p)$ denotes the color of $p$ in $i$-th view. This metric shows the complexity of light change in the observation area. When considering variations in lighting, the angle metric \( H_{\text{ang}} \) additionally takes into account the minimum angle between the vectors formed by the co-visible point \( p \) with the pseudo-view \( I^i_p \) and any source view. Similarly, the resolution metric \( H_{\text{res}} \) additionally considers the minimum difference in distances from the co-visible point \( p \) to the pseudo-view \( I^i_p \) and any source view.

\begin{equation}\label{eq3}
\left\{
\begin{aligned}
H^p_{res} &= \exp\left(-\tan\left(\frac{\pi}{2} \cdot (1 - H^p_{geo})\right) \cdot \min_{o^i_s \in \boldsymbol{I_s}} d^s_p\right), \\
d^s_p &= \max \left(0, \frac{\|o^i_s - p\|_2 - \|o^i_p - p\|_2}{\|o^i_s - p\|_2}\right).
\end{aligned}
\right.
\end{equation}

\begin{equation}\label{eq2}\begin{aligned}H^p_{ang}=\exp\left(-\tan{(\frac{\pi}{2}\cdot (1-H^p_{geo}))}\cdot\min_{o^i_s\in \boldsymbol{I_s}}\angle{o^i_ppo^i_s}\right).\end{aligned}\end{equation}




Let \( M^i_p \) represent the point cloud under the pseudo-view \( I^i_p \), and let \( o_s \) and \( o_p \) denote the coordinates of the source viewpoint and the pseudo-view point, respectively. $d^s_p$ denotes the distance difference between the pseudo-viewpoints and the source viewpoints to the co-visible point, which describes the resolution disparity. The comprehensive metric $V^i_p$ for the final view $I^i_p$ can be expressed as the product of the average values of each term:

\begin{equation}\label{eq4}\begin{aligned} V^i_p = \overline{H^i_{\text{geo}}} \cdot \overline{H^i_{\text{res}}} \cdot \overline{H^i_{\text{ang}}}.\end{aligned}\end{equation}

The overall process is shown in Algorithm~\ref{RFC}.

%===============================pseudo code==============================%
\begin{algorithm}
\caption{Renderability Field Construction}
\begin{algorithmic}

\State \textbf{Input:} Point cloud $\boldsymbol{M}$, images $\boldsymbol{I}$, camera poses $\boldsymbol{T}$, intrinsic parameters $\boldsymbol{K}$
\State \textbf{Output:} Pseudo-view poses $\boldsymbol{T_p}$, metrics $\boldsymbol{V_p}$

\State \textbf{Step 1:} $\boldsymbol{P_v} \gets$ Compute view points using Eq.\ref{view sampling};

\State \textbf{Step 2:} Assign six pseudo-views per viewpoint with orthogonal lines of sight;

\State \textbf{Step 3:} \textbf{for each} image $I_j \in \boldsymbol{I}$ \textbf{and} point $p \in \boldsymbol{M}$: \\
    \hspace{1em} Record color and mark image $I_j($Eq.~\ref{source_img}$)$;

\State \textbf{Step 4:} \textbf{for each} pseudo-view $I^i_p$: \\
    \hspace{1em} $\boldsymbol{M^i_p} \gets \mathbf{F}(\boldsymbol{M}, T^i_p)$; \Comment{Select point cloud in view~\cite{40}} \\
    \hspace{1em} \textbf{for each} point $p \in \boldsymbol{M^i_p}$: \\
    \hspace{2em} $(H^p_{\text{geo}}, H^p_{\text{res}}, H^p_{\text{ang}}) \gets$ Compute metrics with Eq.~\ref{eq1},~\ref{eq3},~\ref{eq2}; \\
    \hspace{1em} \textbf{if} Observation-Conflict($T^i_p$, $\boldsymbol{T_s}$, $\boldsymbol{M^i_p}$) \textbf{then continue}; \\
    \hspace{1em} Compute mean of $\boldsymbol{H^i_{\text{geo}}}, \boldsymbol{H^i_{\text{res}}}, \boldsymbol{H^i_{\text{ang}}}$; \\
    \hspace{1em} $V^i_p \gets$ Metric of pseudo-view $I^i_p$ using Eq.~\ref{eq4};

\end{algorithmic}
\label{RFC}
\end{algorithm}

\subsection{Point Projection Image Restoration}

Image restoration models often depend on contextual inference to fill vacant regions but lack 3D spatial awareness, which hampers geometric consistency. Additionally, noise in the initial image impacts the restoration model’s outcomes. Including low-quality pseudo-views in training can further degrade the reconstructed scene.

Point projection images, derived from discrete 3D points, inherently ensure geometric consistency and multi-view generalizability, thus reducing the difficulty of obtaining wide-baseline view information. Therefore, we use the point projection image as the initial input. We train the Nonlinear Activation Free Network (NAFNet)~\cite{21}, a deep learning model designed for image restoration, to infer RGB images from the point projection images. NAFNet is easy to train and deploy and highly effective for this task.

During training, since inputs comprise discrete points (as shown in Figure~\ref{fig_8} (b)), we treat these images as noise-laden, using the actual captured image as a reference to learn the mapping from the noisy point projection image to the real image, following a denoising task.

In the inference stage, we use the pseudo-view pose obtained previously to render the point projection image, then apply the model to infer the corresponding color image, as shown in Figure~\ref{fig_8} (d). This output consistently preserves scene geometry and weakly textured regions.



\subsection{Staged Gaussian Primitive Optimization}\label{batch}
the restoration quality improves from a new perspective in low-frequency texture regions(e.g. the rounded box region in Figure~\ref{fig_8}). However, due to the limited recovery capability of NAFNet, high-frequency texture cannot be accurately recovered in pseudo-view, and the quality of these regions further degrades when inferred from new perspectives. To address this, we propose a refining strategy in two stages to mitigate the effects of pseudo-views.

In the first stage, we mix all the data and treat the pseudo-view as a noisy ground truth (GT) view, using its angular information to approximate the properties of Gaussian primitives with a high learning rate to better match the actual observations. In this process, the pseudo-view is restricted from guiding the densification operation, as blurred textures could lead to an unintended merging of geometric primitives. 

In the second stage, we fine-tune using only the real images to recover geometric edges and textures by optimizing the spherical harmonic and freezing other elements. As a result, the overall training loss function is similar to vanilla GS, which is defined as follows:
\begin{equation}\label{eq5}
 \mathcal{L} = \lambda_{rgb} \mathcal{L}_1(\hat{I}_i, I_i) + \lambda_{ssim} \mathcal{L}_{ssim}(\hat{I}_i, I_i),
\end{equation}

where $\mathcal{L}_1$ is the photometric loss and $\mathcal{L}_{ssim}$ is the structural similarity loss.
\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{sec/images/image_restoration.pdf}
\caption{Point cloud image restoration. (a) is the ground truth, (b) is the point cloud image from the viewpoint aligned with the ground truth, (c) the restored image corresponding to the point cloud image in the ground truth view, and (d) the restored image from a new wide baseline viewpoint. The four images on the right display zoomed-in regions, highlighted within the orange boxes in images (a) through (d).}
\label{fig_8}
\end{figure}
%add 

==> sec/4_experiments.tex <==

\section{Experiments}
\subsection{Methods of Comparison}
\indent In this paper, we compare our method with five methods known for enhancing model generalization. Among them, CoR-GS~\cite{42} leverages the inconsistency across multiple renderings as a regularization term, while DNGaussian~\cite{3} addresses geometric deviations using depth and normal vectors to ensure geometric consistency in novel viewpoints. SparseGS~\cite{6} improves model generalization by incorporating pseudo-view supervision via pre-trained diffusion models during training. FSGS~\cite{34} enhances the rendering quality of unseen views by guiding the densification of Gaussian primitives. Lastly, Octree-GS~\cite{47} maintains well-initialized Gaussian primitives, ensuring high-quality novel view synthesis.


\begin{figure*}[t]
        \centering
	\begin{minipage}[c]{0.24\textwidth}
		\includegraphics[width=\textwidth]{sec/limitation_study/GT.pdf}
		\subcaption{GT}
		\label{GT}
	\end{minipage}
	\begin{minipage}[c]{0.24\textwidth}
		\includegraphics[width=\textwidth]{sec/limitation_study/vanilla GS.pdf}
		\subcaption{Vanilla GS \cite{2}}
		\label{Baseline}
	\end{minipage} 
	\begin{minipage}[c]{0.24\textwidth}
		\includegraphics[width=\textwidth]{sec/limitation_study/CORGS.pdf}
		\subcaption{CoR-GS \cite{42}}
		\label{CoR}
	\end{minipage}
 	\begin{minipage}[c]{0.24\textwidth}
		\includegraphics[width=\textwidth]{sec/limitation_study/DNGGS.pdf}
		\subcaption{DNGaussian \cite{3}}
		\label{DNGgaussian}
	\end{minipage}
 
  	\begin{minipage}[c]{0.24\textwidth}
		\includegraphics[width=\textwidth]{sec/limitation_study/SparseGS.pdf}
		\subcaption{SparseGS \cite{6}}
		\label{Sparse-GS}
	\end{minipage}
   	\begin{minipage}[c]{0.24\textwidth}
		\includegraphics[width=\textwidth]{sec/limitation_study/FSGS.pdf}
		\subcaption{FSGS \cite{34}}
		\label{FSGS}
	\end{minipage}
        \begin{minipage}[c]{0.24\textwidth}
		\includegraphics[width=\textwidth]{sec/limitation_study/Octree-GS.pdf}
		\subcaption{Octree-GS \cite{47}}
		\label{Octree-GS}
	\end{minipage}
        \begin{minipage}[c]{0.24\textwidth}
		\includegraphics[width=\textwidth]{sec/limitation_study/RF-GS.pdf}
		\subcaption{RF-GS (Ours)}
		\label{RF-GS}
	\end{minipage}

	\caption{View synthesis on the synthetic data. The view is a top view, which differs significantly from the training view. As revealed in comparisons of our model to other GS methods, RF-GS produces more realistic results. Our method mitigates the problems of incomplete, blurring, and numerous artifacts present in new-view synthesis across wide baselines.}
	\label{limitation fig}
\end{figure*}

\begin{table*}[t]
\centering
\caption{Quantitative results on synthetic data. 13 views were evenly separated from all captures for narrow baseline assessment, while 5,449 views were intensively sampled from the scenes. Optimal results are in bold, with secondary results underlined.}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} c|cccc|cccc }
\hline
\multicolumn{1}{l|}{} & \multicolumn{4}{c|}{13 views}                                       & \multicolumn{4}{c}{5,449 views}                                         \\
Method                & PSNR $\uparrow$        & SSIM $\uparrow$         & LPIPS $\downarrow$         & SDP $\downarrow$         & PSNR $\uparrow$         & SSIM $\uparrow$         & LPIPS $\downarrow$         & SDP $\downarrow$         \\ \hline
Vanilla GS~\cite{2}            & \textbf{34.3} & \uline{0.963}          & \uline{0.116}          & \uline{2.26}          & \uline{29.67}          & \uline{0.927}          & \uline{0.174}          & 4.97          \\
CoR-GS~\cite{42}                & \uline{34.29}         & \textbf{0.964} & \textbf{0.113} & \textbf{2.04} & 28.68          & 0.921          & \textbf{0.171}          & 6.12          \\
DNGaussian~\cite{3}                & 30.22         & 0.943          & 0.177          & 2.36          & 27.4           & 0.908          & 0.22           & 4.62          \\
FSGS~\cite{34}                  & 29.82         & 0.945          & 0.176          & 2.69          & 26.94          & 0.913          & 0.215          & 4.62          \\
SparseGS~\cite{6}             & 28.67         & 0.94           & 0.167          & 3.96          & 27.39          & 0.916          & 0.205          & \uline{4.36}          \\
Octree-GS~\cite{47}             & 33.13         & 0.956          & 0.131          & 2.43          & 28.68          & 0.915          & 0.201          & \textbf{4.27} \\
RF-GS (Ours)           & 33.62         & 0.962          & 0.123          & 2.3           & \textbf{29.97} & \textbf{0.933} & \textbf{0.171} & 4.61          \\ \hline
\end{tabular*}
\label{limitation}
\end{table*}
%分别介绍要对比的方法，就是基于稀疏视图的正则化，插值等不同方法
%并说明MVS方法通过预训练得到场景的深度估计，而在我们的前提条件下，激光雷达点云是必须的，因此不适用于该情况

\subsection{Dataset Collection}
We prepared a diverse set of indoor and outdoor datasets for quality comparisons of novel view synthesis in larger-scale scenes. In these datasets, wide-baseline perspectives frequently show a notable drop in rendering quality, especially in overhead, elevated, and aerial views.

\textbf{The synthetic data} was generated from building models in Blender, using a multi-camera setup to capture 360° views per viewpoint. Point cloud data was obtained by sampling discrete 3D points on the mesh model. The capture path simulates real data acquisition, yielding a point cloud and 104 images, used to validate the training strategy's effectiveness and assess limitations in prior metrics.

\textbf {The real-world data} is categorized into indoor and outdoor scenes. The indoor data originates from ScanNet++~\cite{46}, from which we selected a few of the largest scenes. Outdoor data was collected using a customized mobile LiDAR system with two PandarXT32 LiDAR sensors and four GoPro Hero10 cameras. These data serve to evaluate the effectiveness of the algorithm.

% \textbf{Real-world data} was collected using a mobile scanning system with two PandarXT16 LiDARs and four GoPro Hero10 cameras. Indoor environments are typically more challenging due to large areas of weak texture, limited fields of view, and restricted acquisition paths. Therefore, we prepared three sets of real data from different indoor environments. This data validates the algorithm's robustness under highly noisy data.

\textbf{For test data}, we applied the farthest point sampling (FPS) method to the camera viewpoints in the synthetic dataset, following a standard test-to-training ratio of 1:7 to ensure uniform spatial distribution of test data. Additionally, we used the dense sampling method from Section~\ref{RFC} on the simulated scene with a step size $S=1 m$, resulting in 5,449 images for testing the ground truth of the algorithm's performance. For real-world data, we apply a 1:10 test-to-training ratio to quantify the quality of in-scope novel view synthesis, supplemented with qualitative assessments of out-of-scope perspectives to evaluate rendering stability.


\subsection{Metrics of Evaluation}
%分别介绍PSNR等渲染质量指标
%介绍渲染方差指标
To evaluate our approach, the average peak signal-to-noise ratio (PSNR), structural similarity index measure (SSIM)~\cite{28}, and learned perceptual image patch similarity (LPIPS)~\cite{35} were measured. In addition, we express the generalization of the novel perspective in terms of the standard deviation of the PSNR (SDP) of the test data.

\subsection{Details of Experiments}
%介绍实验设备和相关参数设置，为了公平起见，我们使用激光雷达点云初始化所有baseLine方法，确保输入一致。用以比较算法性能的优劣。
The method was tested on a single NVIDIA RTX 4080S GPU with CUDA 11.8. Pseudo-viewpoint sampling was set to $S=2$ m for simulated data, $S=6$ m for real-world data, and $S=1$ m for the smaller public dataset. NAFNet training parameters follow that in~\cite {21}, and GS model training parameters match~\cite{2}, with 20,000 and 10,000 iterations for hybrid and real images-only data, respectively. All methods were initialized using the LiDAR-generated map to ensure fair, consistent inputs.






==> sec/5_Results.tex <==

\section{Results}

\subsection{Synthetic Data}

\textbf{Limitations of evaluation method.}  As shown in Table~\ref{limitation}, we take the evaluation results from 5,449 views as the ground truth for algorithm performance. Although FSGS outperforms SparseGS in local evaluations, this conclusion does not match the global evaluations, indicating that local evaluation results are unreliable for representing the rendering quality of the whole scene. 

Additionally, the global evaluation indicates that CoR-GS matches Octree-GS in PSNR and outperforms it in SSIM and LPIPS. However, as shown in Figure~\ref{CoR}, CoR-GS produces intolerable artifacts and is noticeably weaker than Octree-GS. Combined with the SDP analysis, CoR-GS demonstrates better rendering quality and stability within the local range. Still, its generalization declines significantly beyond this range, indicating more severe overfitting. 

Since three traditional metrics represent average test values and do not capture quality fluctuations, introducing the SDP. When algorithms show similar performance across these metrics, the SDP helps assess their stability. We propose combining all four metrics using spatially uniform test cases to ensure a reliable evaluation of synthesis quality.

\textbf{Advantages of the proposed.} To support a free-roaming experience, the model must generalize across all possible viewpoints within the scene. Top views, which are not manually captured, differ significantly from source views, amplifying Gaussian primitive misalignment and resulting in artifacts and voids (see Figure~\ref{DNGgaussian}). SparseGS and Octree-GS exhibit lower SDP values, indicating improved generalization due to depth regularization and point cloud maintaining technologies, though they face challenges with underfitting and reduced rendering quality. In contrast, our approach enhances multi-view information with pseudo-views, balancing high rendering quality and generalizability for relatively stable performance across diverse perspectives.

\begin{figure}[htp]
        \centering
	\begin{minipage}[c]{0.23\textwidth}
		\includegraphics[width=\textwidth]{sec/Ablation_study/gt.pdf}
		\subcaption{GT}
		\label{GT}
	\end{minipage}
	\begin{minipage}[c]{0.23\textwidth}
		\includegraphics[width=\textwidth]{sec/Ablation_study/GT_ON;Y.pdf}
		\subcaption{w/o $P$}
		\label{Baseline}
	\end{minipage} 
	\begin{minipage}[c]{0.23\textwidth}
		\includegraphics[width=\textwidth]{sec/Ablation_study/MIXED.pdf}
		\subcaption{w/ $P$}
		\label{Mixed data}
	\end{minipage}
 	\begin{minipage}[c]{0.23\textwidth}
		\includegraphics[width=\textwidth]{sec/Ablation_study/P2GT.pdf}
		\subcaption{(w/ $P$, w/o $P$)}
		\label{2STAGE}
	\end{minipage}

	\caption{Effectiveness of staged optimization. The localized zoomed-in area demonstrates the variation in rendering detail.}
	\label{batch train}
\end{figure}

\textbf{Effectiveness of staged Gaussian primitives optimization.}
Table~\ref{ablation} highlights the effectiveness of our strategy outlined in Section~\ref{batch}. Hybrid data training improves model generalization, achieving the lowest SDP, though with reduced rendering quality compared to the baseline. Figure~\ref{Mixed data} shows that mixed data training yields artifact-free and consistent results, but with an overly smooth appearance, lacking realism in details like light reflections and floor texture. To address this, we fine-tune color with ground truth data, enhancing detail, as shown in Figure~\ref{2STAGE}. This approach achieves superior rendering quality and generalization over the baseline.

\begin{table}[htp]
\centering
\caption{Hybrid data training method. $P$ denotes the pseudo-views, with (w/ $P$, w/o $P$) indicating the use of mixed data in stage one and only real captured data in stage two.}
\begin{tabular}{ccccc}
\hline
Method       & PSNR $\uparrow$        & SSIM $\uparrow$       & LPIPS $\downarrow$        & SDP $\downarrow$        \\ \hline
w/o $P$        & 29.67          & 0.927          & 0.174          & 4.97          \\
w/ $P$         & 28.75          & 0.924          & 0.191          & \textbf{4.52} \\
(w/ $P$, w/o $P$) & \textbf{29.97} & \textbf{0.933} & \textbf{0.171} & 4.61          \\ \hline
\end{tabular}
\label{ablation}
\end{table}

%说一下基于前文提到的局限性，我们后面的实验都怎么做
\begin{figure*}[htp]
        \centering
        \begin{minipage}[c]{0.49\textwidth}
	\begin{minipage}[c]{0.96\textwidth}
		\includegraphics[width=\textwidth]{sec/costom data/class_20241113003817.pdf}
	\end{minipage}
        \vspace{0.5cm}
        
	\begin{minipage}[c]{0.49\textwidth}
		\includegraphics[width=\textwidth]{sec/scannet++/our-scanent_20241112052101.pdf}
	\end{minipage} 
	\begin{minipage}[c]{0.49\textwidth}
		\includegraphics[width=\textwidth]{sec/scannet++/SCANNET-WIDE-LINE-3Dgs_20241112050732.pdf}
	\end{minipage}
 
 	\begin{minipage}[c]{0.49\textwidth}
		\includegraphics[width=\textwidth]{sec/scannet++/SCANENT-WIDE-BASELINE-CORGS_20241112050035.pdf}
	\end{minipage}
  	\begin{minipage}[c]{0.49\textwidth}
		\includegraphics[width=\textwidth]{sec/scannet++/SCANET-WIDEBASELINE-OCTREE-GS_20241112050110.pdf}
	\end{minipage}
 		\subcaption{ScanNet++}
		\label{scannet}
        \end{minipage}
                \begin{minipage}[c]{0.49\textwidth}
	\begin{minipage}[c]{0.96\textwidth}
		\includegraphics[width=\textwidth]{sec/costom data/outdoor_20241113003835.pdf}
	\end{minipage}
         \vspace{0.46cm}
 
	\begin{minipage}[c]{0.49\textwidth}
		\includegraphics[width=\textwidth]{sec/costom data/custom/OUTDOOR-OURS_20241112220520.pdf}
	\end{minipage} 
	\begin{minipage}[c]{0.49\textwidth}
		\includegraphics[width=\textwidth]{sec/costom data/custom/3D-GS-outdoor_20241112221157.pdf}
	\end{minipage}
    
 
 	\begin{minipage}[c]{0.49\textwidth}
		\includegraphics[width=\textwidth]{sec/costom data/custom/COR-GS-OUTDOOR_20241112220605.pdf}
	\end{minipage}
  	\begin{minipage}[c]{0.49\textwidth}
		\includegraphics[width=\textwidth]{sec/costom data/custom/octree_20241113052802.pdf}
	\end{minipage}
  		\subcaption{Custom}
		\label{realworld}
        \end{minipage}

	\caption{View synthesis on real-world data. The top image illustrates the scene along with its renderability field, where color transitions from blue to red indicate increasing renderability values. (a) and (b) show the results of wide-baseline synthesis for various algorithms applied to the corresponding scenes, where no ground truth is provided.}
	\label{real-world}
\end{figure*}

\begin{table*}[t]
\centering
\caption{Quantitative results on real-world data. The test data are sampled at a 1:10 ratio from the source views, yielding 17 samples from the ScanNet++ dataset and 16 from the custom dataset. The optimal results are marked in bold, and the secondary results are underlined.}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} c|cccc|cccc }
\hline
\multicolumn{1}{l|}{}          & \multicolumn{4}{c|}{ScanNet++}                                                                                                           & \multicolumn{4}{c}{Custom}                                                                                                           \\
Method                         & PSNR $\uparrow$                               & SSIM $\uparrow$                      & LPIPS $\downarrow$                              & SDP $\downarrow$                                & PSNR $\uparrow$                      & SSIM $\uparrow$                            & LPIPS $\downarrow$                              & SDP $\downarrow$                               \\ \hline
CoR-GS~\cite{42}                         & 25.93                              & \textbf{0.876}            & 0.192                              & 2.7                          &  17.28               & {\ul0.485}                           & {\ul 0.471}                        & 1.73                              \\
DNGaussian~\cite{3}                         & 24.56          & 0.85  & 0.257          & {\textbf{2.17}} & 16.96 & 0.463       & 0.505          & {\ul 1.03} \\
FSGS~\cite{34}                           & 24.71          & 0.856 & 0.245          & {\ul 2.65}          & 16.28 & 0.452       & 0.581          & 1.05   \\
SparseGS~\cite{6}   & \textemdash{}                   & \textemdash{}          & \textemdash{}                   & \textemdash{}                   & \textemdash{}          & \textemdash{}                & \textemdash{}                   & \textemdash{}                  \\
Octree-GS~\cite{47}  & {\textbf{26.24}} & 0.87  & {\textbf{0.171}} & 3.08          & {\ul 17.6}  &  0.469 & {\textbf{0.423}} & \textbf{0.729}         \\
Vanilla GS~\cite{2}                    & 25.93                              & 0.873                     & {\ul 0.191}                        & 2.86                               & 16.65                     & 0.456                           & 0.491                              & 1.21                              \\
RF-GS (Ours)                          & {\ul 25.98}                        & {\ul 0.874}               & 0.215                              & 2.74                               & \textbf{18.49}            & \textbf{0.504}                  & 0.474                              & 1.09                              \\ \hline
\end{tabular*}
\label{real_table}
\end{table*}
\subsection{Real-world Data}
Compared to simulated data, intensive testing is hard to obtain from real-world, so it must be supplemented with qualitative results to evaluate the algorithm's performance. 

ScanNet++ data is relatively dense, so the test data mainly quantifies in-scope view quality and has limited relevance to overall scene generalization. Table~\ref{real_table} indicates that RF-GS performs comparably to standard GS, suggesting that the added pseudo-views did not interfere with source view fitting. Combining with qualitative results, Figure~\ref{scannet} demonstrates that our method significantly enhances challenging regions without introducing noticeable artifacts or voids, outperforming other methods.

The sparse custom data reflects method performance on wide baselines and partially represents generalization across the scene. Table~\ref{real_table} shows that our method achieves minimal distortion, strong geometric consistency, and good stability. As seen in Figure~\ref{realworld}, RF-GS enables stable rendering from any viewpoint, whereas other methods exhibit intolerable blurring in challenging areas.

Notably, SparseGS faced limitations with the number of source views and a narrow baseline requirement, leading to optimization failures and resulting in missing data. More details are available in the appendix.

%真实数据和公开数据各放一组图,然后对应的表格，主要介绍数据集的特点，相比于仿真数据质量如何，每个算法对比有什么特点,包括训练测试数量，伪视图数量

==> sec/6_conclusion.tex <==
\section{Conclusion}

In this paper, we propose a method using renderability fields to enhance generalization in free-scene rendering. First, we introduce a renderability field to guide wide-baseline pseudo-view selection, intensifying supervision. Second, we generate color images from point-projected images via an image restoration model, ensuring both geometric consistency and image quality in pseudo-views. Lastly, hybrid data through staged Gaussian primitives optimization, balancing rendering quality and generalization. Simulation experiments highlight the importance of the generalizability metric, SDP, while comparisons on ScanNet++ and custom datasets demonstrate our approach's superiority over previous work in handling challenging regions.

\textbf{Limitations and Future Works.}The proposed depends on the quality of the pseudo-views; however, when the field of pseudo-view is narrow, the model struggles to correlate image content with the source views, leading to geometric ambiguity at the edges. Therefore, we will consider region-based training to reduce restoration uncertainty.
